On the possible electromagnetic manifestations of merging black holes

We consider scenario of merger of two stellar mass black holes surrounded by an accretion disk. Due to emission of gravitational waves, the mass of the central object decreases and accretion disk experiences perturbation. Calculations show that the main consequence of this disturbance is formation of a shock wave propagating from the center of the disk to its periphery. Light curve is computed and duration of the flash is estimated under assumption that the flash terminates when the luminosity returns to the initial value. It is shown that, if the total mass of the merging binary is 55 M_sol (like in the event GW170814), the flash produced by the shock will increase bolometric luminosity of the disk by 4--6 orders of magnitude, up to 10^{45} erg/s (absolute stellar magnitude -23.8^m). With account of the distance to the source (540 Mpc) and for reasonable assumptions on the parameters of the accretion disk, it turns out that the apparent magnitude of the flash at the maximum of the spectral flux density should be 12.8^m -- 14.2^m, while duration of the flash --- few minutes. The main part of the shock radiation flux is emitted in the X-ray and gamma-ray ranges. In the spectral band of the EPIC instrument of the XMM-Newton observatory or the telescope eROSITA of the Spectrum-RG observatory (0.3--10 keV), luminosity will increase by 3--4 orders of magnitude, up to 10^{44} erg/s, corresponding to the apparent stellar magnitude about 17^m. Luminosity is at maximum in the observational band of the IBIS instrument of the INTEGRAL observatory (20 keV -- 10 MeV) and will be 10^{44} -- 10^{45} erg/s, corresponding to the apparent flux 10^{-4} photons per cm^2/s/keV at the wavelength ~100 keV. From the far UV to the longer wavelengths, the brightening is virtually absent.

==> Makefile <==

OUT := mbbh
TARGET := mbbh


$(TARGET).ps: $(TARGET).dvi
	dvips $(TARGET)

$(TARGET).dvi: $(TARGET).tex #$(TARGET).bbl
	latex $(TARGET)
	latex $(TARGET)

.PHONY: bib bbl
bib bbl: $(TARGET).bbl

$(TARGET).bbl: $(TARGET).bib
	latex $(TARGET)
	bibtex $(TARGET)

.PHONY: pdf
pdf: $(OUT).pdf

$(OUT).pdf: $(TARGET).ps
	ps2pdf $(TARGET).ps $@


.PHONY: zip
zip:
	zip $(OUT).zip Makefile *.eps *.tex *.bib *.sty


.PHONY: clean
clean:
	rm -f *.log *~ $(OUT).pdf $(OUT).zip \
		$(addprefix $(TARGET),.dvi .ps .pdf .aux .log .bbl .blg .out)

